A High School Camp on Algorithms and Coding in Jamaica

This is a report on JamCoders, a four-week long computer-science camp for high school students in Jamaica. The camp teaches college-level coding and algorithms, and targets academically excellent students in grades 9--11 (ages 14--17). Qualitative assessment shows that the camp was, in general terms, a success. We reflect on the background and academic structure of the camp and share key takeaways on designing and operating a successful camp. We analyze data collected before, during and after the camp and map the effects of demographic differences on student performance in camp. We conclude with a discussion on possible improvements on our approach.

==> name.tex <==
 \author{Daniel T. Fokum}
 \authornote{}
 \orcid{0000-0002-9252-3786}
 \affiliation{
   \institution{The University of the West Indies}
   \streetaddress{Mona}
   \city{Kingston}
   \postcode{Kingston 7}
   \country{Jamaica}
 }
 \email{daniel.fokum@uwimona.edu.jm}

 \author{Zaria Chen Shui}
 \authornote{}
 \orcid{0009-0006-2173-2595}
 \affiliation{
   \institution{University of the West Indies, Mona}
   \department{Department of Computing}
   \city{Kingston} 
   \country{Jamaica}
 }
 \email{zaria.chenshui@mymona.uwi.edu}

 \author{Gunjan Mansingh}
 \authornote{}
 \orcid{0000-0002-9252-3786}
 \affiliation{
   \institution{The University of the West Indies}
   \department{Department of Computing}
   \city{Mona} 
   \country{Jamaica} 
   \postcode{1876}
 }
 \email{gunjan.mansingh@uwimona.edu.jm}

 \author{Daniel N. Coore}
\affiliation{%
  \institution{The University of the West Indies}
  \department{Department of Computing}
  \city{Mona} 
  \country{Jamaica} 
}
\email{daniel.coore@uwimona.edu.jm}
